Computation of scattering resonances in absorptive and dispersive media with applications to metal-dielectric nano-structures

In this paper we consider scattering resonance computations in optics when the resonators consist of frequency dependent and lossy materials, such as metals at optical frequencies. The proposed computational approach combines a novel $hp$-FEM strategy, based on dispersion analysis for complex frequencies, with a fast implementation of the nonlinear eigenvalue solver NLEIGS. Numerical computations illustrate that the pre-asymptotic phase is significantly reduced compared to standard uniform $h$ and $p$ strategies. Moreover, the efficiency grows with the refractive index contrast, which makes the new strategy highly attractive for metal-dielectric structures. The $hp$-refinement strategy together with the efficient parallel code result in highly accurate approximations and short runtimes on multi processor platforms.

==> img/backup/SCD/performance_csd.tex <==
\begin{figure}[t]
\centering
%\begin{tikzpicture}[scale=0.75]
%  \begin{loglogaxis}[
%    title={\textsf{TM-cdisk\_r8\_g0\_p2} $\sigma=1.5-0.02i$},
%    ylabel={Time [s]},
%    grid=major,%no markers,
%    log basis x=2,
%    xtick={1,2,4,8,16,32,64,128},
%    xticklabels={1,2,4,8,16,32,64,128},
%    ticklabel style={font=\small},
%    legend style={at={(.98,.98)},anchor=north east,cells={anchor=west},font=\small}
%    ]
%    \addplot coordinates {
%%          (  1,  )
%          (  2,  2.2408e+03)
%          (  4,  1.3706e+03)
%          (  8,  7.2064e+02)
%          ( 16,  4.1257e+02)
%          ( 32,  2.7878e+02)
%          ( 64,  2.0709e+02)
%          (128,  2.3135e+02)
%    };
%    %\legend{tirant}
%  \end{loglogaxis}
%\end{tikzpicture}
\begin{tikzpicture}[scale=0.75]
  \begin{loglogaxis}[
    title={\textsf{TM, $r=8$, $p_0=2$}},
    ylabel={Time [s]},
    grid=major,%no markers,
    log basis x=2,
    xtick={1,2,4,8,16,32,64,128},
    xticklabels={1,2,4,8,16,32,64,128},
    ticklabel style={font=\small},
    legend style={at={(.98,.98)},anchor=north east,cells={anchor=west},font=\small}
    ]
    \addplot coordinates { 
          (  1,  3.9590e+03)
          (  2,  9.8398e+02)
          (  4,  6.5973e+02)
          (  8,  3.7497e+02)
          ( 16,  2.3655e+02)
          ( 32,  1.7228e+02)
          ( 64,  1.4078e+02)
          (128,  1.4852e+02)
    };
    %\legend{nev=50}
  \end{loglogaxis}
\end{tikzpicture}
\hspace{3mm}
%\begin{tikzpicture}[scale=0.75]
%  \begin{loglogaxis}[
%    title={\textsf{TM-cdisk\_r3\_P30\_p10} $\sigma=1.5-0.02i$},
%    ylabel={Time [s]},
%    grid=major,%no markers,
%    log basis x=2,
%    xtick={1,2,4,8,16,32,64,128},
%    xticklabels={1,2,4,8,16,32,64,128},
%    ticklabel style={font=\small},
%    legend style={at={(.98,.98)},anchor=north east,cells={anchor=west},font=\small}
%    ]
%    \addplot coordinates {
%          (  1, 1.4610e+02 )
%          (  2, 7.7533e+01 )
%          (  4, 4.5832e+01 )
%          (  8, 2.4089e+01 )
%          ( 16, 1.4666e+01 )
%          ( 32, 9.0506e+00 )
%          ( 64, 8.0009e+00 )
%          (128, 1.2604e+01 )
%    };
%    %\legend{tirant}
%  \end{loglogaxis}
%\end{tikzpicture}
\begin{tikzpicture}[scale=0.75]
  \begin{loglogaxis}[
    title={\textsf{TM, $r=3$, $p_0=10$}},
    ylabel={Time [s]},
    grid=major,%no markers,
    log basis x=2,
    xtick={1,2,4,8,16,32,64,128},
    xticklabels={1,2,4,8,16,32,64,128},
    ticklabel style={font=\small},
    legend style={at={(.98,.98)},anchor=north east,cells={anchor=west},font=\small}
    ]
    \addplot coordinates { 
          (  1, 7.2342e+01 )
          (  2, 4.3065e+01 )
          (  4, 2.6399e+01 )
          (  8, 1.4087e+01 )
          ( 16, 8.7583e+00 )
          ( 32, 5.7665e+00 )
          ( 64, 5.2629e+00 )
          (128, 8.1390e+00 )
    };
    %\legend{nev=50}
  \end{loglogaxis}
\end{tikzpicture}
\\[2mm]
%\begin{tikzpicture}[scale=0.75]
%  \begin{loglogaxis}[
%    title={\textsf{TE-cdisk\_r8\_g0\_p2} $\sigma=1.5-0.02i$ $nev=8$},
%    ylabel={Time [s]},
%    grid=major,%no markers,
%    log basis x=2,
%    xtick={1,2,4,8,16,32,64,128},
%    xticklabels={1,2,4,8,16,32,64,128},
%    ticklabel style={font=\small},
%    legend style={at={(.98,.98)},anchor=north east,cells={anchor=west},font=\small}
%    ]
%    \addplot coordinates {
%          (  1,  3.2239e+03)
%          (  2,  7.7415e+02)
%          (  4,  5.3244e+02)
%          (  8,  2.8192e+02)
%          ( 16,  1.9515e+02)
%          ( 32,  1.4986e+02)
%          ( 64,  1.2856e+02)
%          (128,  1.2981e+02)
%    };
%    %\legend{tirant}
%  \end{loglogaxis}
%\end{tikzpicture}
\hspace{0.3mm}
\begin{tikzpicture}[scale=0.75]
  \begin{loglogaxis}[
    title={\textsf{TE, $r=8$, $p_0=2$}},
    ylabel={Time [s]},
    grid=major,%no markers,
    log basis x=2,
    xtick={1,2,4,8,16,32,64,128},
    xticklabels={1,2,4,8,16,32,64,128},
    ticklabel style={font=\small},
    legend style={at={(.98,.98)},anchor=north east,cells={anchor=west},font=\small}
    ]
    \addplot coordinates { 
%          (  1,  )
          (  2, 1.9624e+03 )
          (  4, 1.3223e+03 )
          (  8, 6.4399e+02 )
          ( 16, 4.0866e+02 )
          ( 32, 2.5364e+02 )
          ( 64, 1.9569e+02 )
          (128, 2.0276e+02 )
    };
    %\legend{nev=50}
  \end{loglogaxis}
\end{tikzpicture}
\hspace{4.5mm}
%\begin{tikzpicture}[scale=0.75]
%  \begin{loglogaxis}[
%    title={\textsf{TE-cdisk\_r3\_P30\_p10} $\sigma=1.5-0.02i$ $nev=8$},
%    ylabel={Time [s]},
%    grid=major,%no markers,
%    log basis x=2,
%    xtick={1,2,4,8,16,32,64,128},
%    xticklabels={1,2,4,8,16,32,64,128},
%    ticklabel style={font=\small},
%    legend style={at={(.98,.98)},anchor=north east,cells={anchor=west},font=\small}
%    ]
%    \addplot coordinates {
%          (  1,  4.6484e+01)
%          (  2,  3.1451e+01)
%          (  4,  2.0173e+01)
%          (  8,  1.0336e+01)
%          ( 16,  6.4297e+00)
%          ( 32,  4.7202e+00)
%          ( 64,  4.9238e+00)
%          (128,  6.1029e+00)
%    };
%  %   \legend{tirant}
%  \end{loglogaxis}
%\end{tikzpicture}
\begin{tikzpicture}[scale=0.75]
  \begin{loglogaxis}[
    title={\textsf{TE, $r=3$, $p_0=10$}},
    ylabel={Time [s]},
    grid=major,%no markers,
    log basis x=2,
    xtick={1,2,4,8,16,32,64,128},
    xticklabels={1,2,4,8,16,32,64,128},
    ticklabel style={font=\small},
    legend style={at={(.98,.98)},anchor=north east,cells={anchor=west},font=\small}
    ]
    \addplot coordinates { 
          (  1, 1.1644e+02 )
          (  2, 7.6413e+01 )
          (  4, 4.8621e+01 )
          (  8, 2.2261e+01 )
          ( 16, 1.4908e+01 )
          ( 32, 9.6517e+00 )
          ( 64, 9.2191e+00 )
          (128, 1.1252e+01 )
    };
   % \legend{nev=50}
  \end{loglogaxis}
\end{tikzpicture}
\caption{\emph{Parallel execution time (in seconds) of the solver for varying number of MPI processes (up to 128), for problem is \ref{sec:res_CSD}. The target used is $\mu=5.3-0.25i$, where top and bottom plots correspond to TM and TE polariazations respectively. Left plots correspond to a discretization dominant in the $h$-strategy ($r=8$ levels of refinement, polynomial order $p_0=2$), while right plots are for a discretization dominant in the $p$-strategy ($r=3$ levels of refinement, polynomial order $p_0=10$). }}
\label{fig:performance}
\end{figure}





==> img/backup/SCD/table_reference.tex <==
\begin{tabular}{rrS[table-format=2.9, detect-weight]
                  S[table-format=2.9, detect-weight]
                  S[table-format=2.9, detect-weight]
                  S[table-format=2.9, detect-weight] }
\toprule
{$m$} & {$j$} & {$\re \om_{T\!M}$} & {$\im \om_{T\!M}$} & {$\re \om_{T\!E}$} & {$\im \om_{T\!E}$} \\
\midrule
0 & 1  & 1.771128241  & -0.040209598  & 3.028519953  & -0.249632742  \\
1 & 2  & 2.507165546  & -0.308861246  & 1.276108857  & -0.022849842  \\
2 & 3  & 2.637054638  & -0.400052296  & 1.857593240  & -0.103922955  \\
3 & 4  & 3.312034818  & -0.666590209  & 2.444174749  & -0.314200015  \\
4 & 5	 & 3.406691805  & -0.693670033  & 2.506083838  & -0.291213845  \\
5 & 6	 & 3.525244074  & -0.743331707  & 2.324925787  & -0.200153901  \\
6 & 7  & 3.613595702  & -0.818203122  & 3.126303493  & -0.462545189  \\
7 & 8  & 3.671987538  & -0.878964710  & 2.510146419  & -0.300384680  \\
8 & 9  & 3.720376782  & -0.925532212  & 5.549482036  & -0.741472675  \\
9 & 10 & 3.762296208  & -0.963866600  & 3.201508932  & -0.529576832  \\
\bottomrule
\end{tabular}

% TM
% 1.7711282417  -0.0402095986
% 2.5071655468  -0.3088612462
% 2.6370546384  -0.4000522961
% 3.3120348186  -0.6665902090
% 3.4066918050  -0.6936700333
% 3.5252440740  -0.7433317075
% 3.6135957020  -0.8182031229
% 3.6719875384  -0.8789647106
% 3.7203767827  -0.9255322129
% 3.7622962083  -0.9638666004
% 3.7985902462  -0.9961588561

% TE
% 3.0285199537  -0.2496327424
% 1.2761088576  -0.0228498421
% 1.8575932406  -0.1039229554
% 2.4441747496  -0.3142000152
% 2.5060838383  -0.2912138458
% 2.3249257879  -0.2001539019
% 3.1263034939  -0.4625451898
% 2.5101464197  -0.3003846806
% 5.5494820366  -0.7414726751
% 3.2015089320  -0.5295768328
% 3.9127304131  -1.0807566398

  
  
% 3.0285199538  -0.2496327424


==> img/backup/cdimer/table_reference.tex <==
\begin{tabular}{rS[table-format=2.9, detect-weight]
                 S[table-format=2.9, detect-weight]
                 S[table-format=2.9, detect-weight]
                 S[table-format=2.9, detect-weight] }
\toprule
{$j$} & {$\re \om_{T\!M}$} & {$\im \om_{T\!M}$} & {$\re \om_{T\!E}$} & {$\im \om_{T\!E}$} \\
\midrule
 1  &  0.391206696  &  -0.117682733    &  1.275203310  &  -0.017729356 \\
 2  &  0.392635042  &  -0.118062545    &  1.407446763  &  -0.351566607 \\
 3  &  0.809151314  &  -0.171363257    &  1.518834290  &  -0.459714126 \\
 4  &  1.775357827  &  -0.032801891    &  1.833732651  &  -0.071556523 \\
 5  &  2.553994710  &  -0.278675516    &  2.122066617  &  -0.294491051 \\
 6  &  2.654205934  &  -0.403812208    &  2.212801536  &  -0.162351126 \\
 7  &  2.889635797  &  -0.420955865    &  2.904693880  &  -0.427303148 \\
 8  &  2.907250975  &  -0.426266060    &  2.905243670  &  -0.423913316 \\
 9  &  3.613338577  &  -0.811314585    &  2.905244289  &  -0.423897437 \\
10  &  3.668597318  &  -0.875944785    &  3.034308619  &  -0.251533276 \\
11  &  4.152064265  &  -0.280206808    &  3.104957066  &  -0.446726774 \\
12  &  4.459080468  &  -0.244143721    &  4.087887349  &  -0.794352424 \\
13  &  5.565335954  &  -0.248309435    &  4.297453212  &  -0.269106228 \\
14  &  5.952378524  &  -0.278171454    &  4.491337149  &  -0.744646034 \\
15  &  6.175153470  &  -0.890257000    &  5.248059111  &  -0.596147639 \\
16  &  6.636767136  &  -0.423048913    &  5.560206560  &  -0.251973018 \\
17  &  6.672655322  &  -0.452937916    &  5.809753794  &  -0.884187579 \\
18  &  7.251741950  &  -0.616774531    &  6.078619602  &  -0.730690710 \\
19  &  8.155796969  &  -0.628012814    &  7.196957492  &  -0.638546672 \\
20  &  8.855927311  &  -0.444228537    &  8.961786233  &  -0.520547479 \\
\bottomrule
\end{tabular}

% TM, converged
%0.3912066968946-0.11768273301170
%0.3926350425630-0.1180625457580
%0.8091513144625-0.17136325709985
%1.77535782790-0.032801891980
%2.55399471019-0.27867551630
%2.6542059342-0.4038122086
%2.88963579739-0.42095586544
%2.9072509750172-0.4262660604887
%3.613338577758-0.81131458528
%3.668597318176-0.87594478564
%4.152064265487-0.280206808639
%4.45908046830-0.244143721756
%5.56533595433-0.248309435878
%5.95237852419-0.27817145491
%6.1751534707-0.89025700089
%6.636767136-0.423048913
%6.67265532216-0.45293791681
%7.25174195000-0.61677453105
%8.15579696935-0.62801281446
%8.85592731155-0.44422853759

% TE
%1.2752033105-0.0177293569
%1.4074467639-0.351566607
%1.5188342901-0.459714126   
%1.83373265177-0.071556523130
%2.122066617-0.294491051
%2.21280153643-0.16235112682
%2.9046938801306-0.4273031485840
%2.9052436707267-0.4239133160041 %2.9077929558149-0.4253423062755
%2.90524428948-0.4238974375832
%3.03430861918-0.25153327613
%3.1049570668-0.4467267748
%4.087887349-0.794352424
%4.2974532123-0.2691062285
%4.4913371497-0.74464603428
%5.2480591116-0.59614763974
%5.56020656069-0.251973018661
%5.80975379495-0.884187579883
%6.07861960248-0.730690710102
%7.1969574921-0.6385466723
%8.96178623376-0.5205474794
%
%4.8525479424-0.60763161739
%5.27934478017-0.258950063322   
%5.2969221868-0.266451976470




% bold example
% {\bftab 19.1590173402} & \bftab -0.63161790252

% color example
%{\color{blue} 19.1590173402}




==> lib.tex <==
% Updating .sty for LaTeX in ubuntu ...
% http://xiaonosekai.wordpress.com/2012/06/21/manual-update-of-latex-packages-on-ubuntu/

%\usepackage[pdftex]{graphicx}
\usepackage{graphicx}
\usepackage{grffile}
%\usepackage{float}
%\usepackage{subfig}
%\usepackage{overpic}
%\usepackage[T1]{fontenc}
%\usepackage[utf8]{inputenc}

%\usepackage{amsfonts}
%\usepackage{amssymb}

%\usepackage{ucs}
\usepackage{amsmath}
\usepackage{txfonts}
\usepackage{courier}
\usepackage{upgreek}
\usepackage[usenames,dvipsnames,svgnames,table]{xcolor}

%\usepackage{unicode-math}
%\setmathfont{XITS Math}
%\setmathfont[version=setB,StylisticSet=1]{XITS Math}

% \DeclareMathAlphabet{\mathpzc}{OT1}{pzc}{m}{it}

\DeclareMathAlphabet{\mathcal}{OMS}{cmsy}{m}{n} % keeps mathcal unchanged
%\usepackage{epstopdf}
\usepackage{url}
%\usepackage{multicol}

% this code defines a \bar that fits all characters
\newcommand{\barx}[1]{\mkern 1.5mu\overline{\mkern-1.5mu#1\mkern-1.5mu}\mkern 1.5mu}


%\usepackage{makeidx}
%\usepackage{natbib}
%\usepackage{arial}

%\usepackage{makeidx}
%\usepackage{soul}

%\bibpunct{[}{]}{,}{a}{}{;}

% not needed when using a4wide
%\voffset = -0.5cm
%\hoffset = -0.5cm
%\topmargin = 0cm
%\oddsidemargin = 1cm
%\evensidemargin = 1cm
%\textwidth = 16.5cm   % en x
%\textheight = 22cm  % en y

%\voffset = 0cm
%\hoffset = -0.5cm
%\topmargin = 20pt
%\oddsidemargin = 18pt
%\textheight = 22.5cm
%\textwidth = 15.5cm

%\pagestyle{empty}% elimina la numeracion de las painas.
\parskip=2mm%Xmm genera un espacio de X mm entre los parrafos.
\parindent=0mm% elimina la sangria.
% \renewcommand{\labelenumi}{\roman{enumi})} % working before!!!!!!!!!!!!!

% removes space in mm (math mode)
\newcommand{\rs}[1]{\hspace{- #1 mm}} 

\newcommand{\dis}{\displaystyle}
\newcommand{\om}{\omega}
\newcommand{\Om}{\Omega}
\newcommand{\Gm}{\Gamma}

\newcommand{\eps}{\varepsilon}

\newcommand{\n}[1]{{\bf #1}}
\newcommand{\nG}[1]{{\boldsymbol #1}}
\newcommand{\ket}[1]{|#1\rangle}
\newcommand{\bra}[1]{\langle#1|}
\newcommand{\braket}[2]{\langle #1|#2 \rangle}

\newcommand{\fr}[2]{\displaystyle\frac{#1}{#2}}
\newcommand{\tfr}[2]{{\footnotesize\tfrac{#1}{#2}}}
\newcommand{\med}{\tfrac{1}{2}}
\newcommand{\quart}{\tfrac{1}{4}}

\newcommand{\av}[1]{ \langle #1\rangle }  %average
\newcommand{\jp}[1]{ \llbracket #1 \rrbracket }  %jump

\newcommand{\vu}[1]{\displaystyle\hat{\mathbf{#1}}} %Vector unitario
% \newcommand{\vx}[1]{\displaystyle\mathbf{#1}} %Vector
\newcommand{\mx}[1]{\displaystyle\mathbb{#1}} % Matrix, reals: R
\newcommand{\mc}[1]{\mathcal{#1}} % Operators, caligrafic
\newcommand{\mf}[1]{\mathfrak{#1}} % gothic, bilinear forms

\newcommand{\suma}{\sum\limits}
\newcommand{\li}[3]{\displaystyle\lim_{ #1 \rightarrow #2} #3}

\newcommand{\dpar}[2]{\displaystyle\frac{\partial #1}{\partial #2}}
\newcommand{\ddpar}[2]{\displaystyle\frac{\partial^2 #1}{\partial #2^2}}
\newcommand{\dtot}[2]{\displaystyle\frac{d #1}{d #2}}
\newcommand{\ddtot}[2]{\displaystyle\frac{d\,^2 #1}{d #2^2}}

% integrals
\newcommand{\ig}[2]{\displaystyle\int_{#2} #1\, d #2 }
\newcommand{\ix}[2]{\displaystyle\int_{#2} #1\, dx }
\newcommand{\is}[2]{\displaystyle\int_{\partial #2} #1\, ds }
\newcommand{\il}[2]{\displaystyle\int_{ #2} #1\, d} % finish with d# manually

\newcommand{\grad}{\displaystyle\nabla} %Gradiente
\newcommand{\lap}{\displaystyle\Delta} %Laplaciano
\renewcommand{\div}{\displaystyle\nabla\cdot} %Divergencia
\newcommand{\rot}{\displaystyle\nabla\times}  %Rotacional

% function analysis
\newcommand{\h}[2]{||#1||_{#2}}  %Hilbert norms
\newcommand{\re}[1]{\Re\!\left\{#1\right\}}
\newcommand{\im}[1]{\Im\!\left\{#1\right\}}

%discretization
\newcommand{\fem}{\gamma} % discretization index

% backslash
\newcommand{\bslash}{\char`\\}


